Automatic Software Diversity in the Light of Test Suites

A few works address the challenge of automating software diversification, and they all share one core idea: using automated test suites to drive diversification. However, there is is lack of solid understanding of how test suites, programs and transformations interact one with another in this process. We explore this intricate interplay in the context of a specific diversification technique called "sosiefication". Sosiefication generates sosie programs, i.e., variants of a program in which some statements are deleted, added or replaced but still pass the test suite of the original program. Our investigation of the influence of test suites on sosiefication exploits the following observation: test suites cover the different regions of programs in very unequal ways. Hence, we hypothesize that sosie synthesis has different performances on a statement that is covered by one hundred test case and on a statement that is covered by a single test case. We synthesize 24583 sosies on 6 popular open-source Java programs. Our results show that there are two dimensions for diversification. The first one lies in the specification: the more test cases cover a statement, the more difficult it is to synthesize sosies. Yet, to our surprise, we are also able to synthesize sosies on highly tested statements (up to 600 test cases), which indicates an intrinsic property of the programs we study. The second dimension is in the code: we manually explore dozens of sosies and characterize new types of forgiving code regions that are prone to diversification.

==> abstract.tex <==
\begin{abstract}
%The availability of multiple variants of a program that provide the same functionality with different implementations, is of great interest for software engineering. 
%Only 
A few works address the challenge of automating software diversification, and they all share one core idea: using automated test suites to drive  diversification.
However, there is is lack of solid understanding of how test suites, programs and transformations interact one with another in this process. 
We explore this intricate interplay in the context of a specific diversification technique called ``sosiefication''.

Sosiefication generates sosie programs, i.e., variants of a program in which some statements are deleted, added or replaced but still pass the test suite of the original program. 
Our investigation of the influence of test suites on  sosiefication  exploits the following observation:  test suites cover the different regions of  programs in very unequal ways.
Hence, we hypothesize that sosie synthesis has different performances on a statement that is covered by one hundred test case and on a statement that is covered by a single test case.
We synthesize \nbsosies sosies on \nbprograms popular open-source Java programs.
Our results show that there are two dimensions for diversification.
The first one lies in the specification:  the more test cases cover a statement, the more difficult it is to synthesize sosies. Yet, to our surprise, we are also able to synthesize sosies on highly tested statements (up to 600 test cases), which indicates an intrinsic property of the programs we study.
The second dimension is in the code: we manually explore dozens of sosies and characterize new types of forgiving code regions that are prone to diversification.
\end{abstract}



%We have shown that
%- 




% We believe that our findings based on a specific diversification technique -- sosiefication -- can be applied to diversification in general.
% Our results show that there are two dimensions for diversification.
% The first one lies in the specification. There are specification parts that are plastic.
% The literature has already identified some such as video compression, in this paper we propose a new one based on hashing function. But we are convinced that there are many other such plastic specifications. \emph{Future research has to build a comprehensive catalog of plastic behavior.}
% 
% The second dimension is in the code. The forgiving regions parts in the code are those that can be easily modified while maintaining acceptable behavior.
% Often, the implementation of plastic specifications are forgiving (such as the implementation of a video codec). 
% However, this is not a bijection. In our manual analysis, we have encountered forgiving statements in zone that are every conventionally binary in their specification. \emph{There is a need for research on the intersection of plastic behavior and forgiving regions.}
